Reducing Overestimation Bias in Multi-Agent Domains Using Double Centralized Critics

Many real world tasks require multiple agents to work together. Multi-agent reinforcement learning (RL) methods have been proposed in recent years to solve these tasks, but current methods often fail to efficiently learn policies. We thus investigate the presence of a common weakness in single-agent RL, namely value function overestimation bias, in the multi-agent setting. Based on our findings, we propose an approach that reduces this bias by using double centralized critics. We evaluate it on six mixed cooperative-competitive tasks, showing a significant advantage over current methods. Finally, we investigate the application of multi-agent methods to high-dimensional robotic tasks and show that our approach can be used to learn decentralized policies in this domain.

==> include/acronyms.tex <==
%%%%%%%%%%%%%% ACRONYMS %%%%%%%%%%%%%%%%%
\begin{acronym}
	\acro{HRC}{Human-Robot Collaboration}
	\acro{HRT}{Human-Robot Team}
	\acro{RL}{Reinforcement Learning}
	\acro{DRL}{Deep Reinforcement Learning}
	\acro{MARL}{Multi-Agent Reinforcement Learning}
	\acro{DPG}{Deterministic Policy Gradient}
	\acro{DDPG}{Deep Deterministic Policy Gradient}
	\acro{MADDPG}{Multi-Agent Deep Deterministic Policy Gradient}
	\acro{DQN}{Deep Q-Networks}
\end{acronym}


==> include/packages.tex <==
%% include packages for your work in here
\usepackage[colorinlistoftodos]{todonotes}        % for handling TODOs
\usepackage{setspace}
\usepackage{acronym}

